Attack Trees for Security and Privacy in Social Virtual Reality Learning Environments

Social Virtual Reality Learning Environment (VRLE) is a novel edge computing platform for collaboration amongst distributed users. Given that VRLEs are used for critical applications (e.g., special education, public safety training), it is important to ensure security and privacy issues. In this paper, we present a novel framework to obtain quantitative assessments of threats and vulnerabilities for VRLEs. Based on the use cases from an actual social VRLE viz., vSocial, we first model the security and privacy using the attack trees. Subsequently, these attack trees are converted into stochastic timed automata representations that allow for rigorous statistical model checking. Such an analysis helps us adopt pertinent design principles such as hardening, diversity and principle of least privilege to enhance the resilience of social VRLEs. Through experiments in a vSocial case study, we demonstrate the effectiveness of our attack tree modeling with a reduction of 26% in probability of loss of integrity (security) and 80% in privacy leakage (privacy) in before and after scenarios pertaining to the adoption of the design principles.

==> Parallel_Figures/Privacy_In_One.tex <==
\begin{subfigure}[b]{0.50\textwidth}
{
\input{Parallel_Figures/Privacy_Individual.tex}
}
\end{subfigure} 
\begin{subfigure}[b]{0.50\textwidth}
{
\input{Parallel_Figures/Privacy_combinations.tex}
}     
\end{subfigure}
\captionsetup{justification=centering}
\caption{\footnotesize{Vulnerability analysis using the privacy AT}}
\label{fig:S,P-detailed-analysis}

==> Parallel_Figures/Security_In_One.tex <==
\begin{subfigure}[b]{0.50\textwidth}
{
\input{Parallel_Figures/Security_Individual.tex}
}
\end{subfigure} 
\begin{subfigure}[b]{0.50\textwidth}
{
\input{Parallel_Figures/Security_combinations.tex}
}     
\end{subfigure}
\captionsetup{justification=centering}
\caption{\footnotesize{Vulnerability analysis using the security AT}}
\label{fig:S,P-detailed-analysis}

==> STA_Tikz/OR_SAND.tex <==
\begin{subfigure}[b]{0.6\textwidth}
{
\input{STA_Tikz/SAND1.tex}
}
\end{subfigure} 
\begin{subfigure}[b]{0.38\textwidth}
{
\input{STA_Tikz/STA2.tex}
}     
\end{subfigure}
\caption{\footnotesize{STA of a) SAND gate b) leaf node} for security attack tree}
\label{fig:STA-root-leaf}

==> STA_Tikz/STA_Combined.tex <==
\begin{subfigure}[b]{0.38\textwidth}
{
\input{STA_Tikz/STA1.tex}
}
\end{subfigure}
\begin{subfigure}[b]{0.6\textwidth}
{
\input{STA_Tikz/OR1.tex}
}     
\end{subfigure} 
\captionsetup{justification=centering}
\caption{\footnotesize{STA for OR gate and root node of security attack tree.}}
\label{fig:STA-or-leaf}
\vspace{-6.5mm}
%\captionsetup{justification=centering}
%\subcaption{\scriptsize{STA for OR gate with A and B child nodes}}
%\label{fig:Node_A_OR}

==> Tikz_Attack_Trees/Privacy-new.tex <==
\centering
\resizebox{\linewidth}{!}{  
\begin{tikzpicture}[
 % Gates and symbols style
    and/.style={and gate US,thick,draw,fill=red!60,rotate=90,
		anchor=east,xshift=-1mm},
    or/.style={or gate US,thick,draw,fill=blue!60,rotate=90,anchor=east,xshift=-1mm},
% Label style
    label distance=3mm,
    every label/.style={blue},
% Event style
    event/.style={rectangle,thick,draw,fill=yellow!20,text width=2cm,
		text centered,font=\sffamily,anchor=north},
% Children and edges style
    edge from parent/.style={very thick,draw=black!70},
    edge from parent path={(\tikzparentnode.south) -- ++(0,-1.05cm)
			-| (\tikzchildnode.north)},
    level 1/.style={sibling distance=6cm,level distance=1.5cm,
			growth parent anchor=south,nodes=event},
    level 2/.style={sibling distance=5cm, level distance=1.5cm},
    level 3/.style={sibling distance=3cm, level distance=1.5cm},
    level 4/.style={sibling distance=2cm, level distance=1.5cm}
    level 5/.style={sibling distance=2cm, level distance=1.5cm}
%%  For compatability with PGF CVS add the absolute option:
%   absolute
    ]
%% Draw events and edges
\node (g1) [event] {Privacy\\Leakage}
    child[sibling distance=8.5cm]{node (g2) {Location/\\Privacy\\ disclosure}
    child[sibling distance=5.5cm]{node (t1) {Track\\user\\movement}
    child[sibling distance=30mm]{node (s1) {Unauthorized\\access}
    }
    child[sibling distance=20mm, level distance=3cm]{node (s2) {User\\VR space\\location}}
    }
    child[sibling distance=40mm, level distance=2cm]{node (t2){User\\physical\\ location}
    child{node (s3) {Ping\\sweeping}}
    child[level distance=2.3cm]{node (s4) {Capture\\hostname}}
    }
    }
    child[sibling distance=8.5cm]{node(g3){Data/Identity\\ privacy leakage}
    child[sibling distance=12.5mm, level distance=1.5cm]{node (t3) {Capture\\ information
    %Eavesdropping
    }
    child[level distance=2cm, sibling distance=16mm]{node (s5) {Packet\\sniffing}
    child[sibling distance=30mm]{node (l1) {Capture\\packets}}
    child[sibling distance=40mm, level distance=2.5cm]{node (l2) {Analyze\\packets}}
    }
    child[sibling distance=80mm]{node (s6) {Attack\\scenario}
    child[sibling distance=18mm]{node (l3) {Intrusion}}
    child[sibling distance=50mm]{node (l4) {Eavesdropping}}
    }
    }
    child[sibling distance=75mm]{node (t4) {Disclosure\\of sensitive\\information}
    }
    };
%% Place gates and other symbols
%% In the CVS version of PGF labels are placed differently than in PGF 2.0
%% To render them correctly replace '-20' with 'right' and add the 'absolute'
%% option to the tikzpicture environment. The absolute option makes the 
%% node labels ignore the rotation of the parent node.
    \node [or] at (g1.south) [] {};
    \node [or] at (g2.south) [] {};
    \node [and] at (g3.south)(g3) [] {};
        \draw[>=latex,->] (g3.north) to (g3.south);
    %\node [or] at (g3.south) [] {};
    \node [and] at (t1.south)(t1) [] {};
        \draw[>=latex,->] (t1.north) to (t1.south);
    \node [or] at (t3.south) [] {};
    %\node [or] at (t2.south) [] {};
    \node [and] at (t2.south) (t2) [] {};
       \draw[>=latex,->] (t2.north) to (t2.south);
    \node [and] at (s5.south) (s5) [] {};
        \draw[>=latex,->] (s5.north) to (s5.south);
    \node [and] at (s6.south) (s6) [] {};
        \draw[>=latex,->] (s6.north) to (s6.south);
    %\node [or] at (s4.south) [] {};
    %\node [or] at (s7.south) [] {};
\end{tikzpicture}}
\caption{\footnotesize{Privacy AT with privacy leakage as goal}}
\vspace{-2mm}
\label{fig:AT2}


==> Tikz_Attack_Trees/Privacy.tex <==
\centering
    \begin{adjustbox}{width=0.7\textwidth}
\begin{tikzpicture}[
 % Gates and symbols style
    and/.style={and gate US,thick,draw,fill=red!60,rotate=90,
		anchor=east,xshift=-1mm},
    or/.style={or gate US,thick,draw,fill=blue!60,rotate=90,anchor=east,xshift=-1mm},
% Label style
    label distance=3mm,
    every label/.style={blue},
% Event style
    event/.style={rectangle,thick,draw,fill=yellow!20,text width=2.5cm,
		text centered,font=\sffamily,anchor=north},
% Children and edges style
    edge from parent/.style={very thick,draw=black!70},
    edge from parent path={(\tikzparentnode.south) -- ++(0,-1.05cm)
			-| (\tikzchildnode.north)},
    level 1/.style={sibling distance=6cm,level distance=1.5cm,
			growth parent anchor=south,nodes=event},
    level 2/.style={sibling distance=5cm, level distance=1.5cm},
    level 3/.style={sibling distance=3cm, level distance=1.5cm},
    level 4/.style={sibling distance=2cm, level distance=1.5cm}
    level 5/.style={sibling distance=2cm, level distance=1.5cm}
%%  For compatability with PGF CVS add the absolute option:
%   absolute
    ]
%% Draw events and edges
\node (g1) [event] {Privacy Leakage}
    child[level distance=1.3cm, sibling distance=8.5cm]{node (g2) {Location/ Privacy disclosure}
    child[sibling distance=5.5cm, level distance=1.4cm]{node (t1) {Track user movement}
    child[level distance=1.3cm, sibling distance=30mm]{node (s1) {Unauthorized access}
    }
    child[sibling distance=26mm, level distance=1.9cm]{node (s2) {User VR space location}}
    }
    child[sibling distance=40mm, level distance=1.3cm]{node (t2){User physical location}
    child[sibling distance=30mm, level distance=1.3cm]{node (s3) {Ping sweeping}}
    child[sibling distance=30mm, level distance=1.3cm]{node (s4) {Capture hostname}}
    }
    }
    child[level distance=1.3cm, sibling distance=8.5cm]{node(g3){Data / Identity privacy leakage}
    child[sibling distance=12.5mm, level distance=1.3cm]{node (t3) {Capture information}
    child[level distance=1.2cm, sibling distance=16mm]{node (s5) {Packet sniffing}
    child[level distance=1.3cm, sibling distance=48mm]{node (l1) {Capture Packets}}
    child[sibling distance=10mm, level distance=1.3cm]{node (l2) {Analyze packets}}
    }
    child[level distance=1.3cm, sibling distance=70mm]{node (s6) {Attack scenario}
    child[sibling distance=16mm]{node (l3) {Intrusion}}
    child[sibling distance=48mm]{node (l4) {Eavesdropping}}
    }
    }
    child[level distance=1.3cm, sibling distance=75mm]{node (t4) {Disclosure of sensitive information}
    }
    };
%% Place gates and other symbols
%% In the CVS version of PGF labels are placed differently than in PGF 2.0
%% To render them correctly replace '-20' with 'right' and add the 'absolute'
%% option to the tikzpicture environment. The absolute option makes the 
%% node labels ignore the rotation of the parent node.
    \node [or] at (g1.south) [] {};
    \node [or] at (g2.south) [] {};
    \node [and] at (g3.south)(g3) [] {};
        \draw[>=latex,->] (g3.north) to (g3.south);
    %\node [or] at (g3.south) [] {};
    \node [and] at (t1.south)(t1) [] {};
        \draw[>=latex,->] (t1.north) to (t1.south);
    \node [or] at (t3.south) [] {};
    %\node [or] at (t2.south) [] {};
    \node [and] at (t2.south) (t2) [] {};
       \draw[>=latex,->] (t2.north) to (t2.south);
    \node [and] at (s5.south) (s5) [] {};
        \draw[>=latex,->] (s5.north) to (s5.south);
    \node [and] at (s6.south) (s6) [] {};
        \draw[>=latex,->] (s6.north) to (s6.south);
    %\node [or] at (s4.south) [] {};
    %\node [or] at (s7.south) [] {};
\end{tikzpicture}
\end{adjustbox}
\caption{\footnotesize{Attack tree for privacy factors of VRLE case study viz., vSocial}}
\label{fig:AT2}


==> Tikz_Attack_Trees/Security-new.tex <==
\centering
\resizebox{\textwidth}{!}{ 
\begin{tikzpicture}[
 % Gates and symbols style
    and/.style={and gate US,thick,draw,fill=red!60,rotate=90,
		anchor=east,xshift=-1mm},
    or/.style={or gate US,thick,draw,fill=blue!60,rotate=90,anchor=east,xshift=-1mm},
% Label style
    label distance=3mm,
    every label/.style={blue},
% Event style
    event/.style={rectangle,thick,draw,fill=yellow!20,text width=2 cm,text centered,font=\sffamily,anchor=north},
% Children and edges style
    edge from parent/.style={very thick,draw=black!70},
    edge from parent path={(\tikzparentnode.south) -- ++(0,-1.05cm)
			-| (\tikzchildnode.north)},
    level 1/.style={sibling distance=6cm,level distance=1.5cm,
			growth parent anchor=south,nodes=event},
    level 2/.style={sibling distance=5cm, level distance=1.5cm},
    level 3/.style={sibling distance=3cm, level distance=1.5cm},
    level 4/.style={sibling distance=2cm, level distance=1.5cm}
    level 5/.style={sibling distance=2cm, level distance=1.5cm}
%%  For compatability with PGF CVS add the absolute option:
%   absolute
    ]
%% Draw events and edges
\node (g1) [event] {LOI}
    child[sibling distance=8cm]{node (g2) {System \\ compromise}
    child[sibling distance=5.5cm]{node (t1) {Access to\\system}
    child[sibling distance=30mm, level distance=1.5cm]{node (s1) {Unauthorized\\access}
    child{node (l1) {Impersonat\\-ion}}
    child{node (l2) {User\\login}}
    }
    child[sibling distance=48mm, level distance=3.5cm]{node (s2) {Valid \\ access}
    child[level distance=2cm, sibling distance=30mm]{node (l5) {Password \\ attacks}}
    child[level distance=2cm, sibling distance=30mm]{node (l6) {Unauthorized \\ login}}
    }
    }
    child[sibling distance=45mm, level distance=1.5cm]{node (t2){DoS attack\\ initiated}
    child[level distance=1.5cm, sibling distance=20mm]{node (s3) {Packet\\spoofing}}
    child[level distance=3cm, sibling distance=20mm]{node (s4) {Sync\\flood}}
    }}
    child[sibling distance=8cm]{node(g3){Data\\tampering}
    child[sibling distance=30mm, level distance=1.5cm]{node (t3) {Tampered VR space}
    child[level distance=1.5cm, sibling distance=30mm]{node (s5) {SQL injection}}
    child[sibling distance=30mm]{node (s6) {Insert malicious scripts}}
    }
    child{node (t4) {User data tampering}
    child[level distance=3.5cm, sibling distance=20mm]{node (s7) {Packet sniffing}
    child[level distance=1.5cm, sibling distance=40mm]{node (l3) {Capture packets}}
    child[level distance=1.5cm]{node (l4) {Analyze packets}}
    }
    child[sibling distance=30mm]{node (s8) {Modify sensitive data}}
    }
    };
%% Place gates and other symbols
%% In the CVS version of PGF labels are placed differently than in PGF 2.0
%% To render them correctly replace '-20' with 'right' and add the 'absolute'
%% option to the tikzpicture environment. The absolute option makes the 
%% node labels ignore the rotation of the parent node.
    \node [or] at (g1.south) [] {};
    \node [and] at (g2.south)(g2) [] {};
        \draw[>=latex,->] (g2.north) to (g2.south);
    \node [or] at (g3.south) [] {};
    \node [or] at (t1.south) [] {};
    \node [or] at (t2.south) [] {};
    \node [and] at (t3.south) (t3) [] {};
        \draw[>=latex,->] (t3.north) to (t3.south);
    \node [and] at (t4.south) (t4) [] {};
        \draw[>=latex,->] (t4.north) to (t4.south);
    \node [and] at (s1.south) (s1) [] {};
        \draw[>=latex,->] (s1.north) to (s1.south);
    \node [or] at (s2.south) [] {};
    %\node [or] at (s4.south) [] {};
    \node [and] at (s7.south) [] {};
\end{tikzpicture}}
%\end{adjustbox}
\caption{\footnotesize{Security AT with loss of integrity as goal}}
\vspace{-2mm}
\label{fig:AT1}

==> Tikz_Attack_Trees/Security.tex <==
\centering
    \begin{adjustbox}{width=0.7\textwidth}
\begin{tikzpicture}[
 % Gates and symbols style
    and/.style={and gate US,thick,draw,fill=red!60,rotate=90,
		anchor=east,xshift=-1mm},
    or/.style={or gate US,thick,draw,fill=blue!60,rotate=90,anchor=east,xshift=-1mm},
% Label style
    label distance=3mm,
    every label/.style={blue},
% Event style
    event/.style={rectangle,thick,draw,fill=yellow!20,text width=2.7cm,text centered,font=\sffamily,anchor=north},
% Children and edges style
    edge from parent/.style={very thick,draw=black!70},
    edge from parent path={(\tikzparentnode.south) -- ++(0,-1.05cm)
			-| (\tikzchildnode.north)},
    level 1/.style={sibling distance=6cm,level distance=1.5cm,
			growth parent anchor=south,nodes=event},
    level 2/.style={sibling distance=5cm, level distance=1.5cm},
    level 3/.style={sibling distance=3cm, level distance=1.5cm},
    level 4/.style={sibling distance=2cm, level distance=1.5cm}
    level 5/.style={sibling distance=2cm, level distance=1.5cm}
%%  For compatability with PGF CVS add the absolute option:
%   absolute
    ]
%% Draw events and edges
\node (g1) [event] {LOI}
    child[level distance=1.29cm, sibling distance=8cm]{node (g2) {System compromise}
    child[level distance=1.3cm, sibling distance=6.5cm]{node (t1) {Access to system}
    child[sibling distance=55mm, level distance=1.3cm]{node (s1) {Unauthorized access}
    child[sibling distance=36mm]{node (l1) {Impersonation}}
    child[sibling distance=30mm]{node (l2) {User login}}
    }
    child[sibling distance=36mm, level distance=2.1cm]{node (s2) {Valid access}
    child[level distance=1.5cm, sibling distance=30mm]{node (l5) {Password attacks}}
    child[level distance=1.5cm, sibling distance=30mm]{node (l6) {Unauthorized login}}
    }
    }
    child[sibling distance=50mm, level distance=1.3cm]{node (t2){DoS attack initiated}
    child[level distance=1.3cm, sibling distance=20mm]{node (s3) {Packet spoofing}}
    child[level distance=2.2cm, sibling distance=20mm]{node (s4) {Sync flood}}
    }}
    child[level distance=1.3cm, sibling distance=8cm]{node(g3){Data tampering}
    child[sibling distance=30mm, level distance=1.3cm]{node (t3) {Tampered VR space}
    child[level distance=1.3cm, sibling distance=30mm]{node (s5) {SQL injection}}
    child[level distance=1.3cm, sibling distance=30mm]{node (s6) {Insert malicious scripts}}
    }
    child{node (t4) {User data tampering}
    child[level distance=2.2cm, sibling distance=20mm]{node (s7) {Packet sniffing}
    child[level distance=1.5cm, sibling distance=40mm]{node (l3) {Capture packets}}
    child[level distance=1.5cm]{node (l4) {Analyze packets}}
    }
    child[level distance=1.2cm, sibling distance=30mm]{node (s8) {Modify sensitive data}}
    }
    };
%% Place gates and other symbols
%% In the CVS version of PGF labels are placed differently than in PGF 2.0
%% To render them correctly replace '-20' with 'right' and add the 'absolute'
%% option to the tikzpicture environment. The absolute option makes the 
%% node labels ignore the rotation of the parent node.
    \node [or] at (g1.south) [] {};
    \node [and] at (g2.south)(g2) [] {};
        \draw[>=latex,->] (g2.north) to (g2.south);
    \node [or] at (g3.south) [] {};
    \node [or] at (t1.south) [] {};
    \node [or] at (t2.south) [] {};
    \node [and] at (t3.south) (t3) [] {};
        \draw[>=latex,->] (t3.north) to (t3.south);
    \node [and] at (t4.south) (t4) [] {};
        \draw[>=latex,->] (t4.north) to (t4.south);
    \node [and] at (s1.south) (s1) [] {};
        \draw[>=latex,->] (s1.north) to (s1.south);
    \node [or] at (s2.south) [] {};
    %\node [or] at (s4.south) [] {};
    \node [and] at (s7.south) [] {};
\end{tikzpicture}
\end{adjustbox}
\caption{\footnotesize{Attack tree for security factors of VRLE case study viz., vSocial}}
\label{fig:AT1}

==> Tikz_Attack_Trees/SubAT.tex <==
\begin{subfigure}[b]{0.5\textwidth}
{
\input{Tikz_Attack_Trees/Security-new.tex}
}
\end{subfigure} 
\begin{subfigure}[b]{0.48\textwidth}
{
\input{Tikz_Attack_Trees/Privacy-new.tex}
}     
\end{subfigure}
\captionsetup{justification=centering}
\caption{\footnotesize{Attack trees for security and privacy of VRLE case study viz., vSocial}}
%\caption{\footnotesize{}}
\label{fig:STA-root-leaf}

==> Tikz_Code/Design_Princ_Privacy.tex <==
\begin{subfigure}[b]{0.48\textwidth}     
\centering
\resizebox{\linewidth}{!}{
\input{Tikz_Code/Privacy_Unauth_Access.tex}
}
\captionsetup{justification=centering}
\caption{\footnotesize{Pr of disruption on privacy leakage reduced by 68\% as diversity is applied}}  
%on unauthorized access node
\label{Privacy_Defence_Auth}     
\end{subfigure} 
\begin{subfigure}[b]{0.48\textwidth}
\centering
\resizebox{\linewidth}{!}{
\input{Tikz_Code/Privacy_Least_Privilege.tex}
}       
\captionsetup{justification=centering}
%Pr of disruption on privacy leakage reduced to x\% when diversity is applied on unauthorized access
\caption{\footnotesize{Pr of disruption on privacy leakage reduced by 4\% as principle of least privilege is applied}}  
% on eavesdropping node
\label{Privacy_Defence_Redirect}     
\end{subfigure} 
\captionsetup{justification=centering}
\caption{\footnotesize{Effect on probability of disruption of privacy leakage due to application of design principles}}
%\caption{\footnotesize{A before and after Scenario of the Design principles implemented on the tweaked privacy attack tree to show the change in probability of disruption for the root node(privacy leakage).}}
\label{Privacy_Big_Figure}


==> Tikz_Code/Design_Princ_Security.tex <==
\begin{subfigure}[b]{0.48\textwidth}
{
\input{Tikz_Code/Security_Hardening.tex}
}
\end{subfigure} 
\begin{subfigure}[b]{0.48\textwidth}
{
\input{Tikz_Code/Privacy_Diversity_New.tex}
}     
\end{subfigure}
\captionsetup{justification=centering}
\caption{\footnotesize{%Effect on Probability of disruption 
Pr of LoI and privacy leakage due to application of design principles}}
\label{fig:Security_Big_Graph}

==> Tikz_Code/SecNPrivacy_After_Both_Defence.tex <==
\begin{subfigure}[b]{0.48\textwidth}     
\centering
\resizebox{\linewidth}{!}{
\input{Tikz_Code/Security_All_Defence.tex}
}
\captionsetup{justification=centering}
\caption{\footnotesize{$Pr$ of disruption of LoI reduced to 80\% when \{hardening, principle of least privilege\} are employed.}}  
\label{Security_All_Defence}     
\end{subfigure} 
\begin{subfigure}[b]{0.48\textwidth}
\centering
\resizebox{\linewidth}{!}{
\input{Tikz_Code/Privacy_All_Defence.tex}
}       
\captionsetup{justification=centering}
\caption{\footnotesize{$Pr$ of disruption of privacy leakage reduced to 70\% as \{diversity, principle of least privilege\} are employed.}}  
\label{Privacy_All_Defence}     
\end{subfigure}     
\captionsetup{justification=centering}
\caption{\footnotesize{Effect on probability of disruption of goal nodes due to combination of design principles.}}
\label{All_Defence_Big_Figure}

==> Tikz_Upto_section6/Security_Privacy_Time10.tex <==
\begin{subfigure}[b]{0.50\textwidth}
{
\input{Tikz_Upto_section6/security_Time10.tex}
}
\end{subfigure} 
\begin{subfigure}[b]{0.50\textwidth}
{
\input{Tikz_Upto_section6/Privacy_Time10.tex}
}     
\end{subfigure}
\captionsetup{justification=centering}
\caption{\footnotesize{Detailed analysis of one of the most vulnerable TS combinations in security, privacy AT}}
\label{fig:S,P-detailed-analysis}
